Universal Codes for the Gaussian MAC via Spatial Coupling

We consider transmission of two independent and separately encoded sources over a two-user binary-input Gaussian multiple-access channel. The channel gains are assumed to be unknown at the transmitter and the goal is to design an encoder-decoder pair that achieves reliable communication for all channel gains where this is theoretically possible. We call such a system \emph{universal} with respect to the channel gains. Kudekar et al. recently showed that terminated low-density parity-check convolutional codes (a.k.a. spatially-coupled low-density parity-check ensembles) have belief-propagation thresholds that approach their maximum a-posteriori thresholds. This was proven for binary erasure channels and shown empirically for binary memoryless symmetric channels. It was conjectured that the principle of spatial coupling is very general and the phenomenon of threshold saturation applies to a very broad class of graphical models. In this work, we derive an area theorem for the joint decoder and empirically show that threshold saturation occurs for this problem. As a result, we demonstrate near-universal performance for this problem using the proposed spatially-coupled coding system.

==> sensor_reachback.tex <==

\ifpreamble
\newcommand{\defhighlighter}[3][]{%
  \tikzset{every highlighter/.style={color=#2, fill opacity=#3, #1}}%
}

\defhighlighter{yellow}{.5}

\newcommand{\highlight@DoHighlight}{
  \fill [ decoration = {random steps, amplitude=1pt, segment length=15pt}
        , outer sep = -15pt, inner sep = 0pt, decorate
        , every highlighter, this highlighter ]
        ($(begin highlight)+(0,8pt)$) rectangle ($(end highlight)+(0,-3pt)$) ;
}

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \tikzset{this highlighter/.style={#1}}%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable \tikz[overlay, remember picture]
    \highlight@EndHighlight ;%
  }%
  \SOUL@ } 
\makeatother 
\else
\begin{tikzpicture}[>=stealth,auto]
\path[use as bounding box] (-2,-5) rectangle (8,4.5);
\node (a) at (0,0.5) [circle,fill=blue] {};
\node (b) at (1,0) [circle,fill=blue] {};
\node (c) at (2,-1) [circle,fill=blue] {};
\node[left] at (c.west) {$\scriptstyle U_i$};
\node (d) at (1,2) [circle,fill=blue] {};
\node (e) at (2,1) [circle,fill=blue] {};
\node (f) at (0.5,2.5) [circle,fill=blue] {};
\node (g) at (1.3,-2.2) [circle,fill=blue] {};
\node<1-2>[blue] (sensors) at (0,-1) {sensors};

\node<2-> (r) at (7,1) [circle,fill=black] {};
\node<2>[blue] (rec) at (7,0) {collector node};
\draw<2->[->,thick,gray] (a) -- (r); 
\draw<2->[->,thick,gray] (b) -- (r);
\begin{pgfonlayer}{foreground}
\draw<2->[->,thick,gray] (c) -- (r)
node[very near start,sloped,above,black] {$\scriptstyle X_i$}
node[very near end,sloped,above,black] {$\scriptstyle Y_i$};
\end{pgfonlayer}
\draw<2->[->,thick,gray] (d) -- (r);
\draw<2->[->,thick,gray] (e) -- (r);
\draw<2->[->,thick,gray] (f) -- (r);
\draw<2->[->,thick,gray] (g) -- (r);

\node<3->[cloud,aspect=0.6,draw=red,fit=(a) (b) (c) (d) (e)] (fit) {};
\node<3->[blue] (text) at (6,-1.8) {i.i.d. draws from $S$ \highlight[opacity=0.3]{correlated}};
\node<3->[blue] (eq) at (6,-2.3) {\highlight[opacity=0.3]{sources} $\sim \; \Pr(X_1,X_2,\cdots,X_S)$};
\draw<3->[->,very thick,red] (text) -- (fit);
\node<4-5>[blue] (channel) at (6,3) {limited transmission and};
\node<4-5>[blue] (indep) at (6,2.5) {processing capabilities};
\draw<4-5>[->,very thick,red] (indep) -- (1,1);
\draw<5>[thick,gray] (a) -- node[midway,cross out,draw,color=red,sloped,below=-1mm] {} (d);
\node<6->[blue] (q) at (6,-2.8) {\highlight[opacity=0.3]{with independent encoding}};

\node<7->[blue] (channel) at (6,3) {$S$ memoryless channels};
\node<7->[blue] (indep) at (6,2.5) {$\Pr(Y_1^S \mid X_1^S)$ - \highlight[opacity=0.3]{interference}};
\node<7->[blue] (tmp) at (6,2) {\highlight[opacity=0.3]{at receiver}};

\node<8->[blue] (dec) at (7,0) {joint decoding};
%\node (ref) at (1,-3.15) {\cite{barros2003}};
\end{tikzpicture}
\fi
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../slides/presentation"
%%% End: 

